The need for the Higgs boson in the Standard Model

We review the role of the Higgs boson in preserving unitarity of the scattering amplitudes in the Standard Model (SM). We will look at the processes $\nu_e + \bar{\nu}_e \rightarrow W^-_L +W^+_L $, $ W^-_L + W^+_L \rightarrow W^-_L +W^+_L $ and $e^- + e^+ \rightarrow W^-_L +W^+_L $ for longitudinally polarized gauge bosons. Special emphasis will be put in using algebraic methods to evaluate the amplitudes and cross sections. This note is based on Lectures given at the IDPASC Schools in Udine (2012) and Braga (2014).

==> Makefile <==
FILENAME=HiggsAndSM
LATEX = latex
BIBTEX = bibtex
PDFLATEX = ps2pdf
DVIPS = dvips
GV = gv
EV = evince
XDVI = xdvi -s 3
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"

PSFILE = HiggsAndSM.ps 
PDFFILE = HiggsAndSM.pdf
DVIFILE = HiggsAndSM.dvi

COPY = if test -r HiggsAndSM.toc; then cp HiggsAndSM.toc HiggsAndSM.toc.bak; fi 
RM = /bin/rm -f

CLEAN=rm -f HiggsAndSM.aux HiggsAndSM.log HiggsAndSM.dvi HiggsAndSM.toc HiggsAndSM.out HiggsAndSM.blg HiggsAndSM.mtc HiggsAndSM.mtc1 HiggsAndSM.rel HiggsAndSM.vrb HiggsAndSM.end HiggsAndSM.idx HiggsAndSM.bbl HiggsAndSM.rel HiggsAndSM.synctex.gz *~ \#*

WARNING=egrep -i "(Reference|Citation).*undefined" HiggsAndSM.log ; true

HELP=cat /home/romao/usr/help/MakeLatex.help

main:	HiggsAndSM.tex dvi

dvi:	$(DVIFILE)
	$(WARNING)

all:	$(PSFILE) $(PDFFILE)
	$(WARNING)  

ps:	$(PSFILE) 
	$(WARNING)

pdf:	$(PDFFILE)
	$(WARNING)  

gv:	$(PSFILE)
	$(GV) $(PSFILE) &
	$(WARNING)

ev:	$(PSFILE)
	$(EV) $(PSFILE) &
	$(WARNING)

xdvi:	$(DVIFILE)
	$(XDVI) $(DVIFILE)
	$(WARNING)


%.dvi:	%.tex
	$(COPY);$(LATEX) $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ;true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	if [  'cmp -s $*.toc $*.toc.bak'  ]; then $(LATEX) $< ; fi
	$(RM) $*.toc.bak

%.ps:	%.dvi
	dvips $< -o $@

%.pdf:	%.ps
	$(PDFLATEX) $<

clean:	
	$(CLEAN)


realclean: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).pdf $(FILENAME).bbl

cleanps: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).bbl

help:
	$(HELP)


